Parity-Aware Byte-Pair Encoding: Improving Cross-lingual Fairness in Tokenization

Tokenization is the first -- and often least scrutinized -- step of most NLP pipelines. Standard algorithms for learning tokenizers rely on frequency-based objectives, which favor languages dominant in the training data and consequently leave lower-resource languages with tokenizations that are disproportionately longer, morphologically implausible, or even riddled with $<UNK>$ placeholders. This phenomenon ultimately amplifies computational and financial inequalities between users from different language backgrounds. To remedy this, we introduce Parity-aware Byte Pair Encoding (BPE), a variant of the widely-used BPE algorithm. At every merge step, Parity-aware BPE applies a fair-max rule that maximizes the compression gain of the currently worst-compressed language, trading a small amount of global compression for cross-lingual parity. We find empirically that Parity-aware BPE reduces tokenization inequality -- operationalized by the Gini coefficient of per-language token costs -- by up to 89% relative to Classical BPE. This comes with negligible impact on global compression rate and no evidence of systematic degradation in downstream LM performance.

==> figs/128k/30lang_balanced_mc4/latex_tables/comprehensive_metrics_table.tex <==
\begin{table}[htbp]
\centering
\caption{Comprehensive Tokenizer Analysis}
\label{tab:comprehensive_metrics}
% Requires \usepackage{makecell} in preamble
\begin{tabular}{lcccccccccccc}
\toprule
Tokenizer & \makecell{Fertility \\ ($\downarrow$)} & \makecell{Vocab \\ Utilization \\ ($\uparrow$)} & \makecell{TTR \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=1) \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=2.5) \\ ($\uparrow$)} & \makecell{Gini \\ ($\downarrow$)} & \makecell{MorphScore \\ Recall \\ ($\uparrow$)} & \makecell{MorphScore \\ Precision \\ ($\uparrow$)} & \makecell{Avg Token Rank \\ ($\downarrow$)} & \makecell{Token Length \\ ($\uparrow$)} & \makecell{Tokens per Line \\ ($\uparrow$)} & \makecell{Comp. Rate \\ ($\uparrow$)} \\
\midrule
Classical & \textbf{4.092} & 67.4\% & 0.0758 & \textbf{0.86} & 0.49 & 0.051 & 0.513 & \textbf{0.429} & 12126.9 & \textbf{3.47} & 37.5 & \textbf{0.0267} \\
Parity-aware & 4.141 & 66.4\% & 0.0726 & 0.85 & \textbf{0.50} & 0.027 & 0.508 & 0.416 & \textbf{10980.7} & 3.38 & \textbf{38.5} & 0.0259 \\
Parity-aware (hybrid) & 4.113 & 66.3\% & 0.0738 & 0.86 & 0.50 & \textbf{0.023} & 0.508 & 0.420 & 11382.7 & 3.43 & 37.9 & 0.0264 \\
Parity-aware (window) & 4.155 & 67.9\% & 0.0748 & 0.85 & 0.50 & 0.029 & 0.507 & 0.418 & 11355.9 & 3.41 & 38.2 & 0.0261 \\
Parity-aware (window+hybrid) & 4.098 & \textbf{68.1\%} & \textbf{0.0764} & 0.86 & 0.49 & 0.027 & \textbf{0.513} & 0.429 & 11861.3 & 3.46 & 37.6 & 0.0266 \\
\bottomrule
\end{tabular}
\end{table}

==> figs/128k/30lang_unbalanced_fineweb2/latex_tables/comprehensive_metrics_table.tex <==
\begin{table}[htbp]
\centering
\caption{Comprehensive Tokenizer Analysis}
\label{tab:comprehensive_metrics}
% Requires \usepackage{makecell} in preamble
\begin{tabular}{lcccccccccccc}
\toprule
Tokenizer & \makecell{Fertility \\ ($\downarrow$)} & \makecell{Vocab \\ Utilization \\ ($\uparrow$)} & \makecell{TTR \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=1) \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=2.5) \\ ($\uparrow$)} & \makecell{Gini \\ ($\downarrow$)} & \makecell{MorphScore \\ Recall \\ ($\uparrow$)} & \makecell{MorphScore \\ Precision \\ ($\uparrow$)} & \makecell{Avg Token Rank \\ ($\downarrow$)} & \makecell{Token Length \\ ($\uparrow$)} & \makecell{Tokens per Line \\ ($\uparrow$)} & \makecell{Comp. Rate \\ ($\uparrow$)} \\
\midrule
BPE & \textbf{3.990} & 67.0\% & 0.0777 & \textbf{0.85} & 0.49 & 0.064 & 0.659 & 0.537 & 11412.2 & 3.60 & 36.4 & 0.0275 \\
PA-BPE & 4.080 & 70.4\% & 0.0819 & 0.84 & 0.49 & 0.007 & 0.671 & 0.539 & 11569.2 & 3.61 & 36.2 & 0.0276 \\
PA-BPE (window) & 4.042 & 71.6\% & \textbf{0.0838} & 0.84 & 0.48 & 0.009 & \textbf{0.677} & 0.546 & 11847.9 & 3.62 & 36.0 & 0.0278 \\
PA-BPE (hybrid) & 4.056 & 69.8\% & 0.0817 & 0.85 & 0.49 & 0.015 & 0.667 & 0.541 & 11686.3 & 3.63 & 36.0 & 0.0278 \\
PA-BPE (hybrid+window) & 4.029 & 70.8\% & 0.0832 & 0.85 & 0.48 & 0.019 & 0.670 & \textbf{0.546} & 11966.0 & \textbf{3.64} & 35.8 & \textbf{0.0279} \\
PA-BPE (ratios) & 4.398 & 64.9\% & 0.0737 & 0.85 & \textbf{0.49} & 0.040 & 0.669 & 0.532 & \textbf{10406.1} & 3.55 & 37.1 & 0.0270 \\
PA-BPE (dev, GPT-4o) & 4.295 & \textbf{72.3\%} & 0.0796 & 0.85 & 0.49 & \textbf{0.007} & 0.468 & 0.270 & 11973.6 & 3.41 & \textbf{38.2} & 0.0262 \\
\bottomrule
\end{tabular}
\end{table}

==> figs/128k/30lang_unbalanced_fineweb2_devsize_ablation/latex_tables/comprehensive_metrics_table.tex <==
\begin{table}[htbp]
\centering
\caption{Comprehensive Tokenizer Analysis}
\label{tab:comprehensive_metrics}
% Requires \usepackage{makecell} in preamble
\begin{tabular}{lcccccccccccc}
\toprule
Tokenizer & \makecell{Fertility \\ ($\downarrow$)} & \makecell{Vocab \\ Utilization \\ ($\uparrow$)} & \makecell{TTR \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=1) \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=2.5) \\ ($\uparrow$)} & \makecell{Gini \\ ($\downarrow$)} & \makecell{MorphScore \\ Recall \\ ($\uparrow$)} & \makecell{MorphScore \\ Precision \\ ($\uparrow$)} & \makecell{Avg Token Rank \\ ($\downarrow$)} & \makecell{Token Length \\ ($\uparrow$)} & \makecell{Tokens per Line \\ ($\uparrow$)} & \makecell{Comp. Rate \\ ($\uparrow$)} \\
\midrule
PA-BPE (N=100) & 3.973 & \textbf{70.8\%} & \textbf{0.0825} & 0.84 & 0.49 & 0.014 & 0.669 & 0.538 & 11604.1 & 3.60 & 36.2 & 0.0277 \\
PA-BPE (N=300) & 4.019 & 70.7\% & 0.0823 & 0.84 & 0.49 & 0.012 & \textbf{0.672} & 0.539 & 11602.3 & 3.60 & 36.2 & 0.0277 \\
PA-BPE (N=997) & 4.080 & 70.4\% & 0.0819 & 0.84 & \textbf{0.49} & \textbf{0.007} & 0.671 & 0.539 & \textbf{11569.2} & 3.61 & \textbf{36.2} & 0.0276 \\
PA-BPE hybrid (N=100) & \textbf{3.967} & 70.1\% & 0.0821 & 0.85 & 0.48 & 0.022 & 0.666 & 0.540 & 11721.6 & 3.63 & 35.9 & \textbf{0.0278} \\
PA-BPE hybrid (N=300) & 4.015 & 70.0\% & 0.0819 & 0.85 & 0.49 & 0.019 & 0.667 & 0.540 & 11691.3 & 3.63 & 36.0 & 0.0278 \\
PA-BPE hybrid (N=997) & 4.056 & 69.8\% & 0.0817 & \textbf{0.85} & 0.49 & 0.015 & 0.667 & \textbf{0.541} & 11686.3 & \textbf{3.63} & 36.0 & 0.0278 \\
\bottomrule
\end{tabular}
\end{table}

==> figs/128k/30lang_unbalanced_fineweb2_window_ablation/latex_tables/comprehensive_metrics_table.tex <==
\begin{table}[htbp]
\centering
\caption{Comprehensive Tokenizer Analysis}
\label{tab:comprehensive_metrics}
% Requires \usepackage{makecell} in preamble
\begin{tabular}{lcccccccccccc}
\toprule
Tokenizer & \makecell{Fertility \\ ($\downarrow$)} & \makecell{Vocab \\ Utilization \\ ($\uparrow$)} & \makecell{TTR \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=1) \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=2.5) \\ ($\uparrow$)} & \makecell{Gini \\ ($\downarrow$)} & \makecell{MorphScore \\ Recall \\ ($\uparrow$)} & \makecell{MorphScore \\ Precision \\ ($\uparrow$)} & \makecell{Avg Token Rank \\ ($\downarrow$)} & \makecell{Token Length \\ ($\uparrow$)} & \makecell{Tokens per Line \\ ($\uparrow$)} & \makecell{Comp. Rate \\ ($\uparrow$)} \\
\midrule
PA-BPE (W=50) & 4.056 & 71.3\% & 0.0832 & 0.84 & \textbf{0.48} & \textbf{0.008} & 0.673 & 0.542 & \textbf{11742.7} & 3.62 & \textbf{36.1} & 0.0277 \\
PA-BPE (W=100) & \textbf{4.042} & \textbf{71.6\%} & \textbf{0.0838} & \textbf{0.84} & 0.48 & 0.009 & \textbf{0.677} & \textbf{0.546} & 11847.9 & \textbf{3.62} & 36.0 & \textbf{0.0278} \\
PA-BPE (W=150) & 4.049 & 71.5\% & 0.0835 & 0.84 & 0.48 & 0.009 & 0.674 & 0.543 & 11799.8 & 3.62 & 36.0 & 0.0277 \\
PA-BPE (W=200) & 4.043 & 71.6\% & 0.0837 & 0.84 & 0.48 & 0.009 & 0.677 & 0.546 & 11842.6 & 3.62 & 36.0 & 0.0278 \\
\bottomrule
\end{tabular}
\end{table}

==> figs/128k/30lang_unbalanced_mc4/latex_tables/comprehensive_metrics_table.tex <==
\begin{table}[htbp]
\centering
\caption{Comprehensive Tokenizer Analysis}
\label{tab:comprehensive_metrics}
% Requires \usepackage{makecell} in preamble
\begin{tabular}{lcccccccccccc}
\toprule
Tokenizer & \makecell{Fertility \\ ($\downarrow$)} & \makecell{Vocab \\ Utilization \\ ($\uparrow$)} & \makecell{TTR \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=1) \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=2.5) \\ ($\uparrow$)} & \makecell{Gini \\ ($\downarrow$)} & \makecell{MorphScore \\ Recall \\ ($\uparrow$)} & \makecell{MorphScore \\ Precision \\ ($\uparrow$)} & \makecell{Avg Token Rank \\ ($\downarrow$)} & \makecell{Token Length \\ ($\uparrow$)} & \makecell{Tokens per Line \\ ($\uparrow$)} & \makecell{Comp. Rate \\ ($\uparrow$)} \\
\midrule
BPE & 4.178 {\small $\pm$ 0.048} & 65.1\% & 0.0718 & \textbf{0.86} & \textbf{0.50} & 0.067 & \textbf{0.527 {\small $\pm$ 0.042}} & \textbf{0.434 {\small $\pm$ 0.045}} & 11288.4 & 3.43 {\small $\pm$ 0.01} & 38.2 {\small $\pm$ 0.1} & 0.0262 \\
UnigramLM & 4.536 {\small $\pm$ 0.041} & 56.3\% & 0.0457 & 0.74 & 0.29 & 0.095 & 0.262 {\small $\pm$ 0.049} & 0.147 {\small $\pm$ 0.035} & \textbf{6605.5} & 2.51 {\small $\pm$ 0.00} & \textbf{51.9 {\small $\pm$ 0.1}} & 0.0193 \\
PA-BPE & 4.138 {\small $\pm$ 0.047} & 66.4\% & 0.0727 & 0.85 & 0.50 & \textbf{0.027} & 0.508 {\small $\pm$ 0.044} & 0.418 {\small $\pm$ 0.048} & 10988.9 & 3.38 {\small $\pm$ 0.00} & 38.5 {\small $\pm$ 0.1} & 0.0260 \\
PA-BPE (hybrid) & \textbf{4.116 {\small $\pm$ 0.048}} & 66.3\% & 0.0737 & 0.86 & 0.50 & 0.027 & 0.515 {\small $\pm$ 0.044} & 0.426 {\small $\pm$ 0.047} & 11370.9 & 3.43 {\small $\pm$ 0.00} & 37.9 {\small $\pm$ 0.1} & 0.0264 \\
PA-BPE (window) & 4.152 {\small $\pm$ 0.048} & 67.9\% & 0.0749 & 0.85 & 0.50 & 0.029 & 0.507 {\small $\pm$ 0.042} & 0.417 {\small $\pm$ 0.046} & 11368.9 & 3.41 {\small $\pm$ 0.00} & 38.2 {\small $\pm$ 0.1} & 0.0262 \\
PA-BPE (window+hybrid) & 4.127 {\small $\pm$ 0.048} & \textbf{67.9\%} & \textbf{0.0761} & 0.86 & 0.49 & 0.031 & 0.517 {\small $\pm$ 0.043} & 0.430 {\small $\pm$ 0.045} & 11785.0 & \textbf{3.46 {\small $\pm$ 0.00}} & 37.6 {\small $\pm$ 0.1} & \textbf{0.0266} \\
\bottomrule
\end{tabular}
\end{table}

==> figs/128k/60lang_unbalanced_mc4/latex_tables/comprehensive_metrics_table.tex <==
\begin{table}[htbp]
\centering
\caption{Comprehensive Tokenizer Analysis}
\label{tab:comprehensive_metrics}
% Requires \usepackage{makecell} in preamble
\begin{tabular}{lcccccccccccc}
\toprule
Tokenizer & \makecell{Fertility \\ ($\downarrow$)} & \makecell{Vocab \\ Utilization \\ ($\uparrow$)} & \makecell{TTR \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=1) \\ ($\uparrow$)} & \makecell{Rényi \\ ($\alpha$=2.5) \\ ($\uparrow$)} & \makecell{Gini \\ ($\downarrow$)} & \makecell{MorphScore \\ Recall \\ ($\uparrow$)} & \makecell{MorphScore \\ Precision \\ ($\uparrow$)} & \makecell{Avg Token Rank \\ ($\downarrow$)} & \makecell{Token Length \\ ($\uparrow$)} & \makecell{Tokens per Line \\ ($\uparrow$)} & \makecell{Comp. Rate \\ ($\uparrow$)} \\
\midrule
BPE & \textbf{3.564 {\small $\pm$ 0.026}} & \textbf{72.8\%} & \textbf{0.0341} & 0.83 & 0.51 & 0.144 & \textbf{0.481 {\small $\pm$ 0.027}} & \textbf{0.335 {\small $\pm$ 0.029}} & 9882.6 & \textbf{3.16 {\small $\pm$ 0.00}} & 45.1 {\small $\pm$ 0.1} & 0.0222 \\
PA-BPE & 3.707 {\small $\pm$ 0.027} & 58.9\% & 0.0264 & 0.83 & \textbf{0.52} & \textbf{0.083} & 0.466 {\small $\pm$ 0.026} & 0.288 {\small $\pm$ 0.027} & \textbf{7534.8} & 2.92 {\small $\pm$ 0.00} & \textbf{47.1 {\small $\pm$ 0.1}} & 0.0212 \\
PA-BPE (hybrid) & 3.624 {\small $\pm$ 0.027} & 60.4\% & 0.0279 & \textbf{0.84} & 0.52 & 0.100 & 0.450 {\small $\pm$ 0.027} & 0.293 {\small $\pm$ 0.027} & 8353.5 & 3.03 {\small $\pm$ 0.00} & 45.7 {\small $\pm$ 0.1} & 0.0219 \\
PA-BPE (window) & 3.647 {\small $\pm$ 0.027} & 70.1\% & 0.0321 & 0.82 & 0.51 & 0.101 & 0.469 {\small $\pm$ 0.026} & 0.314 {\small $\pm$ 0.027} & 8982.6 & 3.05 {\small $\pm$ 0.00} & 46.0 {\small $\pm$ 0.1} & 0.0218 \\
PA-BPE (window+hybrid) & 3.576 {\small $\pm$ 0.027} & 72.1\% & 0.0338 & 0.82 & 0.50 & 0.116 & 0.466 {\small $\pm$ 0.027} & 0.323 {\small $\pm$ 0.027} & 9717.6 & 3.14 {\small $\pm$ 0.00} & 45.0 {\small $\pm$ 0.1} & \textbf{0.0222} \\
\bottomrule
\end{tabular}
\end{table}
